A Forest Mixture Bound for Block-Free Parallel Inference

Coordinate ascent variational inference is an important algorithm for inference in probabilistic models, but it is slow because it updates only a single variable at a time. Block coordinate methods perform inference faster by updating blocks of variables in parallel. However, the speed and stability of these algorithms depends on how the variables are partitioned into blocks. In this paper, we give a stable parallel algorithm for inference in deep exponential families that doesn't require the variables to be partitioned into blocks. We achieve this by lower bounding the ELBO by a new objective we call the forest mixture bound (FM bound) that separates the inference problem for variables within a hidden layer. We apply this to the simple case when all random variables are Gaussian and show empirically that the algorithm converges faster for models that are inherently more forest-like.

==> tex/background.tex <==
{\bf Notation} Vector-valued variables are written in bold. For a variational distribution $q(\bm y | \bm x)$, we denote the expectation over $q$ as $\underset{q}{\mathbb E}[\cdot]$ and the conditional entropy of $\bm y$ given $\bm x$ as $\underset{q}{H} (\bm y | \bm x)$. An \textit{exponential family} of distributions is a family of distributions parameterized by $\eta$ of the form

\begin{align*}
p(x) = \exp \{ g(x) + t(x) \cdot \eta - a(\eta) \} \ , \
\end{align*}
where $g$ is the log-base measure, $t$ are the sufficient statistics, $\eta$ are the natural parameters, and $a$ is the log-partition function.

==> tex/general_case.tex <==
In general, this choice of $u$ and $\alpha$ are not optimal for any exponential family / log-partition function. However, they are optimal and provide tight bounds in two important cases: when $text{Var}[\mathbf y] = 0$, i.e., MAP estimation, and when $p(\mathbf x | \mathbf y)$ is a forest model. 

==> tex/spectral_radius_proof.tex <==
Let's prove this. First will need this lemma: for any square matrix $A$, $\lambda$ is an eigenvalue of $A$ if and only if $1-\lambda$ is an eigenvalue of $I - A$. Proof: let $\lambda$ be an eigenvalue of $A$, and let $\mathbf x$ be the corresponding eigenvector. Then $\mathbf x$ is an eigenvector of $I-A$ with eigenvalue $1-\lambda$:

\[
(I-A) \mathbf x = \mathbf x - A \mathbf x = \mathbf x - \lambda \mathbf x = (1-\lambda) \mathbf x
\]

Similarly, if $1-\lambda$ is an eigenvalue of $I-A$ with eigenvector $\mathbf x$, then $\mathbf x$ is an eigenvector of $A$ with eigenvalue $\lambda$:

\[
A \mathbf x = (A \mathbf x - \mathbf x) + \mathbf x = -(I-A) \mathbf x + \mathbf x = -(1 - \lambda) \mathbf x + \mathbf x = \lambda \mathbf x
\]

So the eigenvalues of $I - D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right)$ are one minus the eigenvalues of $D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right)$. To get $\rho \left( I - D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right) \right) < 1$, we need the eigenvalues of $D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right)$ to be in $(0, 2)$. In fact, we'll show the eigenvalues are in $(0, 1]$.

Let's show that the eigenvalues of $D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right)$ are positive, i.e., that matrix is positive definite. To do this, we will need the following lemma: similar matrices have the same spectrum, and thus the same spectral radius. In detail, for any square matrix $A$ and inverible matrix $S$, $\rho(A) = \rho(S^{-1} AS)$. Proof: If $\mathbf x$ is an eigenvector of $A$ with eigenvalue $\lambda$, then $S^{-1} x$ is an eigenvector of $S^{-1} A S$ with eigenvalue $\lambda$:

\[
S^{-1} A S (S^{-1} \mathbf x) = S^{-1} A \mathbf x = S^{-1} \lambda \mathbf x = \lambda (S^{-1} \mathbf x)
\]

So $A$ has the same spectrum as $S^{-1} A S$ and thus the same spectral radius. Applying this with $S = D^{-1/2}$ and $A = D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right)$, we get that the eigenvalues of $A$ equal the eigenvalues of

\[
D^{-1/2} \left( \frac{1}{\sigma_p^2} I + W^T W \right) D^{-1/2}
\]

Note that $\frac{1}{\sigma_p^2} I + W^T W$ is positive definite, since $W^T W$ is positive semi-definite and so has eigenvalues $\geq 0$, and so $\frac{1}{\sigma_p^2} I + W^T W$ has eigenvalues $\geq \frac{1}{\sigma_p^2} > 0$. We can use another lemma: for any positive-definite matrix $A$ and invertible matrix $S$, $S^T A S$ is positive definite. Proof: for any $\mathbf x \neq 0$, $S \mathbf x \neq 0$ since $S$ is invertible. Then

\[
\mathbf x^T (S^T A S) \mathbf x = (S \mathbf x)^T A (S \mathbf x) > 0
\]

by the positive definiteness of $A$. We can apply this to our matrix: since $D^{-1/2}$ is invertible (and symmetric), $D^{-1/2} \left( \frac{1}{\sigma_p^2} I + W^T W \right) D^{-1/2}$ must be positive definite, and so then must $D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right)$.

Now we need to prove the eigenvalues are $\leq 1$. If we can find a matrix $B$ such that $\|B^{-1} D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right) B\|_\infty \leq 1$, then we can use

\begin{align*}
\rho (D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right)) &= \rho(B^{-1} D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right) B) \\
&\leq \|B^{-1} D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right) B\|_\infty \\
&\leq 1
\end{align*}

In fact, we'll find such a $B$ that is a diagonal matrix, $\text{diag}(\beta)$. Then the sum of the absolute components of row $j^*$ of $B^{-1} D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right) B$ is

\begin{align*}
\beta_{j^*}^{-1} \sigma_{j^*}^2 \left( \beta_{j^*} \frac{1}{\sigma_p^2} + \sum_{j=1}^m \beta_j |w_{j^*} \cdot w_j| \right) &\leq 1 \\
\beta_{j^*} \frac{1}{\sigma_p^2} + \sum_{j=1}^m \beta_j |w_{j^*} \cdot w_j| &\leq \beta_{j^*} \sigma_{j^*}^{-2} \\
&= \beta_{j^*} \left( \frac{1}{\sigma_p^2} + \sum_{i=1}^n \frac{w_{ij^*}^2}{\alpha_{ij^*}} \right) \\
\sum_{j=1}^m \beta_j |w_{j^*} \cdot w_j| &\leq \beta_{j^*} \sum_{i=1}^n \frac{w_{ij^*}^2}{\alpha_{ij^*}} \\
\end{align*}

So now we just need to find that matrix $B$. The following choice satisfies this condition:

\[
\beta_j = \left( \sum_{i=1}^n \frac{w_{ij}^2}{\alpha_{ij}^2} \right)^{-1/2}
\]

Then

\begin{align*}
\beta_{j} \sum_{i=1}^m \frac{w_{ij}^2}{\alpha_{ij}} &= \sum_{i=1}^m \sum_{j'=1}^m \alpha_{ij'} \beta_j \frac{w_{ij}^2}{\alpha_{ij}} \\
&= \sum_{j'=1}^m  \sum_{i=1}^m \alpha_{ij'} \beta_j \frac{w_{ij}^2}{\alpha_{ij}} \\
&= \sum_{j'=1}^m  \beta_j \langle \alpha_{j'} \odot \mathbf w_j, \frac{1}{\alpha_j} \odot \mathbf w_j \rangle \\
\beta_j \sum_{i=1}^m \frac{\alpha_{ij'}}{\alpha_{ij}} |w_{ij}|^2 &\geq \beta_{j'} \sum_{i=1}^n |w_{ij}| |w_{ij'}| \\
\beta_j \langle \alpha_{j'} \odot |w_j|, \frac{1}{\alpha_j} \odot |w_j| \rangle &\geq \beta_{j'} \langle \alpha_{j'} \odot |w_j|, \frac{1}{\alpha_{j'}} \odot |w_{j'}| \rangle \\
\beta_j \langle \alpha_j \odot \alpha_{j'} \odot |\hat w_j|, |\hat w_j| \rangle &\geq \beta_{j'} \langle \alpha_j \odot \alpha_{j'} \odot |\hat w_j|, |\hat w_{j'}| \rangle \\
\beta_j \cos \theta \left[ \alpha_j \odot \alpha_{j'} \odot |\hat w_j|, |\hat w_j| \right] &\geq \beta_{j'} \cos \theta \left[ \alpha_j \odot \alpha_{j'} \odot |\hat w_j|, |\hat w_{j'}| \right] \\
\end{align*}

If $\alpha_{ij} \propto |w_{ij}| \lambda_j$ for some set of $\{\lambda_j\}_{j=1}^m$, e.g., $\lambda_j = \text{Std}[y_j]$, then the inequality holds and the proof is finished.

==> tex/splitting_alg.tex <==
For a fixed $\varepsilon$, the updates to $\mu_j$ can be viewed as the iterates of a certain splitting algorithm for solving the linear system

\[
\left( \frac{1}{\sigma_p^2} I + W^T W \right) \bm y = W^T(\bm x - \bm b)
\]

Or equivalently, optimizing the ridge regression problem

\[
\min_{\bm y} \frac{1}{2} \left\Vert (W \bm y + \bm b) - \bm x \right\Vert_2^2 + \frac{1}{2 \sigma_p^2} \left\Vert \bm y \right\Vert_2^2
\]

We can write the update for $\mu$ as

\begin{align*}
\sigma_j^2 &= \left( \frac{1}{\sigma_p^2} + \sum_{i=1}^n \frac{w_{ij}^2}{\varepsilon_{ij}} \right)^{-1} \\
D &= \text{diag}(\{1/\sigma_j^2\}_{j=1}^m) \\
\mu_{t+1} &= D^{-1} \left[ W^T (\bm x - \bm r) + \left( D - \frac{1}{\sigma_p^2} I \right) \mu_t \right] \\
&= D^{-1} \left[ W^T (\bm x - \bm b) - W^T W \mu_t + \left( D - \frac{1}{\sigma_p^2} I \right) \mu_t \right] \\
&= D^{-1} \left[ W^T (\bm x - \bm b) + \left( D - \left( \frac{1}{\sigma_p^2} I + W^T W \right) \right) \mu_t \right] \\
\end{align*}

From this it is clear that for any stationary point of the iteration $\mu$,

\begin{align*}
\mu &= D^{-1} \left[ W^T (\bm x - \bm b) + \left( D - \left( \frac{1}{\sigma_p^2} I + W^T W \right) \right) \mu \right] \\
D \mu &= W^T (\bm x - \bm b) + \left( D - \left( \frac{1}{\sigma_p^2} I + W^T W \right) \right) \mu \\
0 &= W^T (\bm x - \bm b) - \left( \frac{1}{\sigma_p^2} I + W^T W \right) \mu \\
 \mu &= \left( \frac{1}{\sigma_p^2} I + W^T W \right)^{-1} W^T (\bm x - \bm b) \\
\end{align*}

So $\mu$ is the solution to a certain linear system, and the updates provide an iterate algorithm for finding that solution. In fact, this iterative algorithm can be described by the matrix splitting 

\[
\frac{1}{\sigma_p^2} I + W^T W = D - \left( D - \left( \frac{1}{\sigma_p^2} I + W^T W \right) \right)
\]

To prove that the algorithm converges, we need to show that the update matrix has spectral radius less than $1$:

\[
\rho \left( I - D^{-1} \left( \frac{1}{\sigma_p^2} I + W^T W \right) \right) < 1
\]


